SoK on Performance Bounds in Anonymous Communication

Communicating anonymously comes at a cost - and large communities have been in a constant tug-of-war between the development of faster protocols, and the improvement of security analyses. Thereby more intricate privacy goals emerged and more detailed bounds on the minimum overhead necessary to achieve them were proven. The entanglement of requirements, scenarios, and protocols complicates analysis, and the published results are hardly comparable, due to deviating, yet specific choices of assumptions and goals (some explicit, most implicit). In this paper, we systematize the field by harmonizing the models, comparing the proven performance bounds, and contextualizing these theoretical results in a broad set of proposed and implemented systems. By identifying inaccuracies, we demonstrate that the attacks, on which the results are based, indeed break much weaker privacy goals than postulated, and tighten the bounds along the way. We further show the equivalence of two seemingly alternative bounds. Finally, we argue how several assumptions and requirements of the papers likely are of limited applicability in reality and suggest relaxations for future work.

==> sections/mainAttacks.tex <==
To prove their bounds, the papers design an attack applicable to any protocol (matching their protocol model) and conclude that without a certain amount of overhead the attack cannot be prevented.


\subsubsection{\Gelernter}\label{sec: attack gelernter}
%Here the attacker tries to exclude at least one sender from the set of senders that possibly have sent \emph{all} real messages.  Therefore, the attacker observes how many messages (sum of real and dummy) each sender sends and controls the destination(s) to learn that $\mu_u$ real messages are received. If the sender that sent the least messages has sent less than $\mu_u$ messages, the adversary knows that not all messages are from this sender.
\cite{gelernter2013limits}'s privacy goal requires that all participating senders could have sent \emph{all} real messages. 
The attacker attempts to exclude at least one of them, by counting the number of messages they are sending.
%Providing the scenarios, the adversary chooses a single sender to send all $\mu_u$ real messages.
Knowing the number of real messages that are received, the adversary can exclude any sender who sent less messages. 
%Counting the numbers of sent messages, the adversary aims to exclude at least one of the senders
%Here the attacker tries to exclude at least one sender from the set of senders that possibly have sent \emph{all} real messages.  
%Therefore, the attacker observes how many messages (sum of real and dummy) each sender sends and controls the destination(s) to learn that $\mu_u$ real messages are received. 
%If the sender that sent the least messages has sent less than $\mu_u$ messages, the adversary knows that not all messages are from this sender.
The protocol thus cannot deliver more real messages to corrupt receivers  than any sender sends in real and dummy messages. Since all receivers are considered corrupt, every user has to send as many messages as the protocol can deliver.
% (the adversary can exclude one hypothetical sender of the messages, otherwise). 

Notice that this bound only discusses dummy messages, i.e. bandwidth overhead: Every user has to send as many messages as are received. 



\subsubsection{Trilemma}\label{sec:attackTri}
%The adversary in \cite{das2018anonymity} does not control who generates dummy messages, but only who sends real messages to which receiver.
\cite{das2018anonymity} assumes a corrupted receiver that receives a message and wants to figure out which of two suspected users sent the message. Two ways of identifying the sender are considered.

\emph{The non-compromising\footnote{This name is used to distinguish it from the compromising adversary, even though the non-compromising adversary compromises the receiver.} adversary:}
First, the attacker monitors the sending behavior of both suspected challenge users. If one of them did not send any message (real or dummy) in the $l_{max}$ rounds\footnote{The given number of $l_{max}$ rounds includes the current round, i.e. the round in which the challenge message is received.} before the challenge message is received, the other user must be the sender.

\emph{The compromising adversary:}
The second attack exploits an even worse situation: The adversary is assumed to also control some intermediate nodes. 
First, the adversary can trivially identify the sender if she by chance controls all intermediate nodes on the path of the challenge message.
%If all parties on the challenge message's path are corrupted,  the adversary can track the message and figure out the sender. 
Second, even if she controls only the intermediate nodes on the paths of the cover messages, she can observe that these are not the challenge message, and thus identifies the sender indirectly.
%Further, if all parties on the path of the cover messages, i.e. all messages sent by the other challenge user in the respective time interval, are corrupted, the adversary also knows that the received message is none of them and thus knows the sender.

Notice that against these attacks both higher latency and bandwidth overhead helps, which causes the authors to call the bound Trilemma (as one cannot get strong privacy, low latency and bandwidth cost at the same time):
%To achieve privacy in this setting, a certain latency $l_{max}$ (maximum allowed path length between sender and receiver) or number of dummy messages is requires, and trade-offs between these two strategies are calculated.
Increasing the probability of sending a dummy message translates to a  larger set of candidate users that might have sent the message, and thus a better chance that the alternative suspect is in it. 
Increasing the latency reduces the chance of all intermediate nodes being corrupt, and, also increases the interval during which the message may have been sent, which again translates to a larger set of candidate senders. 

%Increasing the maximal latency $l_{max}$, with all other parameters fixed, decreases the chances of the adversary.
%First, there is more time in which the alternative user can send and extending the paths to more nodes, the likelihood that all are corrupted drops.
%Second, adding dummy messages as bandwidth overhead $\beta$ also hinders the adversary: It increases the chance that the alternative user has sent a (dummy) message in the considered time window.

%In this setting, instead of two messages matrices, the scenarios differ in the sender $u_b$ of he challenge message. The adversary can distinguish the scenarios and win if the protocol invariant is not fulfilled. Te invariant consists of two parts. Firstly, the adversary monitors
%If this is the case, then she chooses her answer $b'$ randomly. If one of the challenge users $u_{b-1}$ has not sent then the adversary knows from which user the challenge message was sent and wins the game.
%Additionally, the setting of compromising adversary is discussed, who can cooperate with some of the nodes in the network that forward the message.Therefore the probability of an adversary to win the game depends on the likelihood that both challenge user send in a given number of rounds, the duration $l_{max}$ a message might spent in the network before being received by the destination and the number of nodes the adversary is allowed to cooperate with.

\subsubsection{\Ando}
\cite{ando2019complexity} assumes an active adversary who wants to figure out which of two suspected senders communicates to the receiver, by dropping messages and observing successful deliveries.
She chooses a candidate sender, drops as many messages sent by this sender as she can, and observes whether an expected message still arrives at the receiver, or not.
She guesses her victim to be the real sender if no message arrives, and the alternative sender if it does.
%In this attack the adversary tries to drop as many packets coming from the victim sender as she is able to. Then the adversary observes whether a message arrives at the receiver that is expected to get a certain message (e.g. the next packet of a message stream). If no message arrives, the adversary concludes that the expected message was sent from the victim and has been dropped.

Notice that both latency and bandwidth overhead help against the attack:
Increasing the number of redundant messages that are relayed over alternative first hops at higher bandwidth cost decreases the chance of all paths being controlled by the adversary, and hence increases the chance of the message to be delivered. %(colliding routes cause a slightly decreased benefit of this strategy).
Higher latency increases the chance of a message that has not been sent by the chosen candidate user to be relayed through her and then dropped by the adversary. This finally reduces the accuracy of the adversary's guess\footnote{Note that this paper assumes an integrated system model, in which users also act as intermediate nodes.}.


%This attack can be hindered with introducing more packets into the network: The sender sends copies of the message over different first hops. If at least one of the first hops is honest (and the routing does not send the packet back to the victim), the message reaches the receiver. Further, it can also be hindered by increasing latency: The attack fails if the message was originally sent by someone else, but routed over the victim, because then the adversary's conclusion that the victim is the sender is wrong. If all packets are routed over more hops, the probability that the critical message is routed over the victim\footnote{Note that this argumentation as well as their proof assumes that users act as intermediate nodes.} increases, just as the latency does.

%The adversary chooses message matrices which satisfy the condition that each user sends  and receives exactly one message. In addition,  the view for each node that is controlled by the attacker must not change between those chosen challenge scenarios, meaning the nodes that cooperate with the adversary have to receive and send the same messages in each scenario. She wins if she can differentiate between two scenarios.
%The adversary then aims to drop as many onions passing corrupted nodes with the message send by a specific user ("Alice") that she can determine the receiver ("Bob") because he receives no (assumption used to conceive the bound) or only few (used in the proposed protocol) onions.

%\subsubsection{Discussion}
%
% On the other hand, the Trilemma and Ando both are influenced by latency and bandwidth. All attacks are very simple ones to optimally work on all protocols. However, we will see some restrictions and grasp the differences in the bounds in the following sections.

\todo[inline]{Should we illustrate the attacks in a figure?}
